SplitSR: An End-to-End Approach to Super-Resolution on Mobile Devices

Super-resolution (SR) is a coveted image processing technique for mobile apps ranging from the basic camera apps to mobile health. Existing SR algorithms rely on deep learning models with significant memory requirements, so they have yet to be deployed on mobile devices and instead operate in the cloud to achieve feasible inference time. This shortcoming prevents existing SR methods from being used in applications that require near real-time latency. In this work, we demonstrate state-of-the-art latency and accuracy for on-device super-resolution using a novel hybrid architecture called SplitSR and a novel lightweight residual block called SplitSRBlock. The SplitSRBlock supports channel-splitting, allowing the residual blocks to retain spatial information while reducing the computation in the channel dimension. SplitSR has a hybrid design consisting of standard convolutional blocks and lightweight residual blocks, allowing people to tune SplitSR for their computational budget. We evaluate our system on a low-end ARM CPU, demonstrating both higher accuracy and up to 5 times faster inference than previous approaches. We then deploy our model onto a smartphone in an app called ZoomSR to demonstrate the first-ever instance of on-device, deep learning-based SR. We conducted a user study with 15 participants to have them assess the perceived quality of images that were post-processed by SplitSR. Relative to bilinear interpolation -- the existing standard for on-device SR -- participants showed a statistically significant preference when looking at both images (Z=-9.270, p<0.01) and text (Z=-6.486, p<0.01).

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/background.tex <==
\section{Background}
\label{sec:background}

Standard convolutional layers are the fundamental building blocks for many computer vision applications. When many convolutional layers are stacked together to form very deep networks, residual connections can be used to facilitate gradient flow through the network during training. At a certain point, many networks become too computationally intensive for on-device systems, especially when the channel dimension of the feature maps is large. Assuming the input and output channels of a given convolutional layer are both $N$, the computational complexity of a standard convolutional layer is $O(N^{2})$. In this section, we will cover recent optimizations of convolutional layers that attempt to reduce convolutional computational complexity while maintaining high accuracy.


\subsection{BottleneckBlock \& ShuffleBlock}
\label{section: bottleneck}


\citet{howard2017mobilenets} proposed the use of depthwise separable convolutions to stack residual blocks and achieve a strong balance between accuracy and latency. These operations, also known as BottleneckBlocks, consist of two parts: a 3$\times$3 depthwise convolution and by a 1$\times$1 pointwise convolution. The depthwise convolution is used to expand features and makes use of single convolutional filters at every input channel to perform lightweight filtering, while the pointwise convolution constructs new features by calculating linear combinations of input channels. Based on the success of BottleneckBlock, ShuffleBlock, introduced by \citet{ma2018shufflenet}, is an advanced version of BottleneckBlocks with several innovations (Figure~\ref{fig:compare_blocks}A). First, ShuffleBlocks use channel-splitting to evenly split the input channels into branches. Only one branch is used for computation, where each channel is processed through two 1$\times$1 pointwise convolutions and one 3$\times$3 depthwise convolution. The branches are then concatenated, after which the channels are shuffled to allow information to be communicated between the two branches. The computation reduction is:

\begin{figure*}[t!]
  \includegraphics[width=\textwidth]{Figures/all_blocks.jpg}
  \caption{Schematics showing several lightweight residual blocks from prior work: (A) ShuffleBlock~\cite{ma2018shufflenet}, (B) IdleBlock~\cite{xu2019hybrid}, and (C) GhostBlock~\cite{han2019ghostnet}.}
  \label{fig:compare_blocks}
\end{figure*}

\begin{equation} \label{eq:shuffleblock}
 \frac{1}{2\times D_{k}\times D_{k}} + \frac{\alpha_{1}}{N}
\end{equation}

where $N$ is the number of channels, D$_{k}$ is the kernel size and $\alpha_{1} \in (0,1]$ is the split ratio for the channel-splitting. In ShuffleNet, Ma et al. used $\alpha_{1} = 0.5$ for an even split.


\subsection{Inverted Residual Block \& IdleBlock}

Inverted residual blocks are designed to process significantly more spatial information during the depthwise convolution. To do this, these blocks add an additional pointwise layer at the beginning to expand low-dimensional information to a high-dimensional representation. After going through the depthwise convolution, these blocks use another pointwise layer to project the high-dimensional representation to the original low-dimensional space. \citet{sandler2018mobilenetv2}, who first proposed these blocks as part of their MobileNetV2 work, gained considerable improvements in top1/top5 performance on the ImageNet dataset. Recently, \citet{xu2019hybrid} proposed the idea of combining an inverted residual block with a ShuffleBlock (without channel-shuffling) in order to prune superfluous connections. This construct, called an IdleBlock (Figure~\ref{fig:compare_blocks}B), has the following computation reduction factor:

\begin{equation} \label{eq:idle}
 \frac{2\beta\alpha_{1}^2}{D_{k}\times D_{k}}+\frac{\alpha_{1}\beta}{N}
\end{equation}
Note that when the expansion ratio $\beta=1$ and the split ratio $\alpha_{1}=0.5$, the computation reduction is the same as the ShuffleBlock. \citet{xu2019hybrid} also studied the use of IdleBlock in various hybrid configurations using two different type of lightweight residual block for image classification and achieved the state-of-the-art accuracy against other mobile-specific neural networks. 

\subsection{GhostBlock}
CNNs often contain redundancy in their feature maps. Calling these redundancies \textit{ghost} features, \citet{han2019ghostnet} recognized this inefficiency as an opportunity for optimization. They proposed the notion of a GhostBlock (Figure~\ref{fig:compare_blocks}C) for generating redundant feature maps with cheap linear operations rather than ordinary convolutions.
Within a GhostBlock, an ordinary convolution kernel is applied to generate a few intrinsic feature maps. Linear operations are used to generate redundant feature maps, which are then stacked with the intrinsic feature maps to produce the block's output. 
When pointwise convolution is used in the GhostBlock's first layer and depthwise convolution is used for cheap linear operations, the reduction in computation is:
\begin{equation}
 \frac{\alpha_{2}}{D_{k}\times D_{k}}+\frac{1-\alpha_{2}}{M}
\end{equation}
where $\alpha_{2}\in (0,1]$ is the fraction of intrinsic feature maps to total feature maps, also known as the squeeze ratio. \\

\noindent
To the best of our knowledge, there is no existing work on applying IdleBlock and GhostBlock to the task of image SR, making us the first to evaluate these techniques in this context. 

